HoPP: Robust and Resilient Publish-Subscribe for an Information-Centric Internet of Things

This paper revisits NDN deployment in the IoT with a special focus on the interaction of sensors and actuators. Such scenarios require high responsiveness and limited control state at the constrained nodes. We argue that the NDN request-response pattern which prevents data push is vital for IoT networks. We contribute HoP-and-Pull (HoPP), a robust publish-subscribe scheme for typical IoT scenarios that targets IoT networks consisting of hundreds of resource constrained devices at intermittent connectivity. Our approach limits the FIB tables to a minimum and naturally supports mobility, temporary network partitioning, data aggregation and near real-time reactivity. We experimentally evaluate the protocol in a real-world deployment using the IoT-Lab testbed with varying numbers of constrained devices, each wirelessly interconnected via IEEE 802.15.4 LowPANs. Implementations are built on CCN-lite with RIOT and support experiments using various single- and multi-hop scenarios.

==> figs/styles.tex <==
\tikzset{
    router/.style = {circle, draw, fill=gray!50, align=center, text centered, node distance=0.95cm,scale=1.2,font=\tiny\sffamily, inner sep=2pt},
    contentproxy/.style = {router, rectangle, fill=red!50},
    tree_building/.pic={
        \node[contentproxy,label={above:CP}] (-CP) {\phantom{0}};
        \node[router, below left of=#1-CP] (-N1) {1};
        \node[router, below right of=#1-CP] (-N2) {2};
        \node[router, below left of=#1-N1] (-N3) {3};
        \node[router, below right of=#1-N1] (-N4) {4};
        \node[router, below right of=#1-N2] (-N5) {5};
    },
    fibelem/.style = {draw=black, align=center, font=\small\sffamily},
    fibth/.style = {fibelem, fill=gray!20},
    fib/.style = {matrix of nodes, text width=2.25em, nodes={fibelem}, text depth=0.01em, text height=.5em},
}

